Implementing Multi-Periodic Critical Systems: from Design to Code Generation

This article presents a complete scheme for the development of Critical Embedded Systems with Multiple Real-Time Constraints. The system is programmed with a language that extends the synchronous approach with high-level real-time primitives. It enables to assemble in a modular and hierarchical manner several locally mono-periodic synchronous systems into a globally multi-periodic synchronous system. It also allows to specify flow latency constraints. A program is translated into a set of real-time tasks. The generated code (\C\ code) can be executed on a simple real-time platform with a dynamic-priority scheduler (EDF). The compilation process (each algorithm of the process, not the compiler itself) is formally proved correct, meaning that the generated code respects the real-time semantics of the original program (respect of periods, deadlines, release dates and precedences) as well as its functional semantics (respect of variable consumption).

==> deadline-calculus.tex <==
\label{sec:deadline-calculus}
In practice we cannot compute separately the adjusted deadline of each
task instance of our task graph, as the instance set is
infinite. Instead, for each task we represent the sequence of deadlines
of its instances as a finite repetitive pattern called
\textit{\dword}. The deadline calculus performs the encoding of task
precedences by computing a \dword\ for each task of the task graph.

% The clock calculus provides additional data
% for schedulability analysis as it gives information on conditional
% execution of tasks. While the actual value of a boolean clock can only
% be computed at execution time, we still know before execution that a
% task $A$ with clock $ck\Onn c$ and a task $B$ with clock $ck\Onnot c$
% will never become schedulable simultaneously. As a consequence, the 

\subsection{Task Deadlines vs Task Instance Deadlines}
Figure \ref{fig:dw-usefull} shows an example that is schedulable with 
set different deadlines for different instances of a task while it is
not when we use the same deadline for every instance of the
task. Indeed, if we set $d_B[n]=6$ for $n\in\mathbb{N}$, $d_A[n]=2$ for
$n\in 2\mathbb{N}$ and $d_A[n]=4$ for $n\in 2\mathbb{N}+1$, the task set
$\{A,\;B\}$ is schedulable: $A[0]$ is scheduled during time interval
$[0,2[$, $B[0]$ during $[4,6[$, $A[1]$ during $[6,8[$ and this schedule
repeats indefinitely. Now, if we set the same deadline for all instances
of $A$, that is $d_{A}[n]=2$ for $n\in\mathbb{N}$, then either $A[1]$ or
$B[0]$ will miss their deadline (the absolute deadline 6). This
motivates the introduction of task \dwords.

\begin{figure}[hbt]
  \centering
  \lstinputlisting[basicstyle=\scriptsize]{dw-usefull.lrt}
  \caption{The instances of $A$ cannot all have the same deadline}
  \label{fig:dw-usefull}
\end{figure}


\subsection{Deadline Words}
A \emph{unitary deadline} specifies the relative deadline for the
computation of a single instance of a task. A unitary deadline is simply
an integer value $d$. An \emph{infinite periodic deadline word}, or
simply a \emph{\dword} defines the sequence of unitary deadlines for
each instance of a task. The set of \dwords\ $\dwset$ is defined by the
following grammar:
\[
\begin{array}{lcl}
  w & ::= & \drepeat{u}\\
  u & ::= & d \Alt d.u\\
\end{array}
\]
$\drepeat{u}$ denotes the infinite repetition of word $u$. $w[n]$
denotes the $n^{th}$ unitary deadline of \dword\ $w$
($n\in\mathbb{N}$). $|u|$ denotes the length of the finite word $u$
(the number of unitary deadlines in $u$). Notice that $\drepeat{u}[n]$
can be efficiently computed as: $\drepeat{u}[n]=u[n\;mod\;|u|]$. The
ordering relation on \dwords\ is the lexicographic order: $ \forall
w_1,w_2\in\dwset,\;w_1\leq w_2\Leftrightarrow \forall i\in
\mathbb{N},\;w_1[i]\leq w_2[i]$. The minimum of two \dwords\
$w_m=min(w_i,w_j)$ is such that for all $n$,
$w_m[n]=min(w_i[n],w_j[n])$. Similarly, the sum of two \dwords\
$w=w_i+w_j$ is such that for all $n$ $w[n]=w_i[n]+w_j[n]$. Finally, the
word $w=w_i+k$, with $w_i\in\dwset$ and $k\in\mathbb{N}$ is such that
for all $n$, $w[n]=w_i[n]+k$.

\subsection{Computing Task Deadline Words}

Let $w_i$ denote the \dword\ representing the sequence of deadlines of
all the instances of task $\tau_i$.  From Sect. \ref{sec:encoding-sync},
we know that each task precedence $\tau_i\precany \tau_j$ can be encoded
as a constraint relating $w_i$ to $w_j$ of the form $w_i\leq
w_j+\diffops_{ops}(T_j)-C_j+r_j-r_i$, where $\diffops_{ops}(T_j)$ is a
word such that $\diffops_{ops}(T_j)[n]=\diffops_{ops}(n,T_j)$ for all
$n$. To be able to compute $\diffops_{ops}(T_j)$, we must prove that it
is a \textit{periodic} word.

\begin{property}
  \label{ppt:diffops-periodic}
  The function $\diffops_{ops}(n,T_j)$ is periodic of period
  $\pword(ops)$, with $\pword(ops)$ defined as follows:
  \begin{itemize}
  \item $\pword(\Emptylist)=1$
  \item $\pword(\List{\Uclock k}(ops))=\pword(ops)/gcd(\pword(ops),k)$
  \item $\pword(\List{\Dclock k}(ops))=k*\pword(ops)$
  \item $\pword(\List{\Phclock q}(ops))=\pword(ops)$
  \end{itemize}
\end{property}
\begin{proof}
  We prove that
  $\diffops_{ops}(n,T_j)=\diffops_{ops}(n+\pword(ops),T_j)$ by induction
  on the structure of $ops$ using the same remarks as for Property
  \ref{ppt:delta-ops}. Notice that we do not prove that $\pword(ops)$ is
  the \textit{smallest} $p$ such that $\diffops_{ops}(n,T_j)$ is periodic of
  period $p$.
\end{proof}

Thanks to this property, $\diffops_{ops}(T_j)$ is indeed a \dword\ and
we can compute it as described in Alg. \ref{alg:cstrops}.
\begin{algorithm}
  \caption{Computing $\diffops_{ops}(T_j)$}
  \begin{algorithmic}[1]
    \State let $w$ be a \dword\ of size $\pword(ops)$
    \For{$cpt$ from 0 to $\pword(ops)-1$}
    \State $w[cpt]=\diffops_{ops}(cpt,T_j)$
    \EndFor
    \State \Return w
  \end{algorithmic}
\label{alg:cstrops}
\end{algorithm}
Then we compute $w_j+\diffops_{ops}(T_j)$ by unfolding $w_j$ and
$\diffops_{ops}(T_j)$ on $lcm(P(ops),|w_j|)$ and by adding the two
results point by point. The value of $w_i$ can finally be computed as the
combination of all the constraints on $w_i$:
$w_i=min(w_i,min(\diffops_{ops}(T_j)+w_j+r_j-r_i-C_j))$ (for all
$\tau_j$, $\tau_i\precany \tau_j$).

We give an algorithm for computing the task \dwords\ of a reduced task
graph in Alg. \ref{alg:deadlines}. For this algorithm, delayed
precedences are removed from the task graph. As a reduced task graph is
a DAG (when we do not consider delayed precedences), the algorithm is
basically a topological sort \cite{kahn62} working backwards, starting
from the end of the graph and computing deadline constraints at each
step. This algorithm is similar to the one presented in \cite{chetto90}
but applied to extended precedences.

\begin{algorithm}
  \caption{Computing task \dwords\ of a reduced task graph}
  \begin{algorithmic}[1]
    \For{Every $\tau_i$}
    \If{$\tau_i$ is an actuator with a constraint ($\tau_i$ \lstinline!due n!)}
    \State $w_i\gets \drepeat{n}$
    \Else \;$w_i\gets \drepeat{T_i}$
    \EndIf
    \EndFor
    \State $S\gets$ List of tasks without successors
    \While{$S$ is not empty}
    \State Remove the head $\tau_j$ of $S$
    \For{Each $\tau_i$ such that $\tau_i\precany\tau_j$ and
      $\Fbyshort\not\in ops$}
    \State $w_i\gets min(w_i,\diffops_{ops}(T_j)+w_j+r_j-r_i-C_j)$
    \State Remove the precedence $\tau_i\precany\tau_j$ from the graph
    \If{$\tau_i$ has no other successor}
    \State Insert $\tau_i$ in $S$
    \EndIf
    \EndFor
    \EndWhile
  \end{algorithmic}
  \label{alg:deadlines}
\end{algorithm}

If we accept programs which contain a precedence $\tau_i\precany\tau_j$
where $ops$ contains an operator $\Uclock k$ that precedes the first
operator $\Fbyshort$ appearing in $ops$ (which we rejected in
Sect. \ref{sec:reduced-graph}), then we can have a delayed precedence
$\tau_i\precany\tau_j$ where $w_i$ depends on $w_j$. As a consequence,
we cannot compute task \dwords\ using a topological sort on tasks, but
instead we must use a topological sort on task instances. This can be
done by unfolding the task graph into a task instance graph. This will
not be detailed here.

\subsection{Correction and Complexity}
Our precedence encoding algorithm satisfies the following properties:
\begin{th-std}
  For all $\tau_i\precany\tau_j$, we have for all $n$,
  $\tau_i[n]\precrel\tau_j[g_{ops}(n)]$. Then we have:
  \[w_i[n]\leq w_j[n]+\diffops_{ops}(w_j)[n]+r_j-r_i-C_j
  \]
\end{th-std}
\begin{proof}
  From the definition of $\diffops_{ops}(w_j)$.
\end{proof}

\begin{property}
  For every $w_i$ computed by Alg. \ref{alg:deadlines}:
  \begin{align}
    |w_i| &= lcm(\{lcm(P(ops),|w_j|),\text{for all
    }\tau_i\precany\tau_j\})\label{subppt:dd-size}\\
    |w_i| &\leq lcm(\{T_k,\text{ for all }\tau_k\})\label{subppt:dd-bound}
  \end{align}
\end{property}
\begin{proof}
  Part \ref{subppt:dd-size} directly comes from the definition of
  $\diffops_{ops}(w_j)$. For part \ref{subppt:dd-bound}, we first prove that for all
  $\tau_i\precany\tau_j$, $P(ops)|T_j$. Let $\pinotinv$ denote the
  inverse of function $\piinv$, ie $T_j=\pinotinv_{ops}(T_i)$. We prove
  by induction that $P(ops)|\pinotinv_{ops}(T_i)$ and so that
  $P(ops)|T_j$. From this property and from part \ref{subppt:dd-size},
  we have $|w_i|\leq lcm(|w_j|,T_j)$. So transitively $|w_i| \leq
  lcm(\{T_k,\text{ for all }\tau_k\})$.
\end{proof}

\begin{property}
  The complexity of Alg. \ref{alg:deadlines} is
  $\mathcal{O}(|V|+|E|*|w_{max}|)$ where $w_{max}$ denotes the \dword\
  which has the longest size in the task graph.
\end{property}
\begin{proof}
  The complexity of a topological sort for a graph $g=(V,E)$ is
  $\mathcal{O}(|V|+|E|)$. Our algorithm performs the same operations as
  a topological sort but in addition at each step (for each edge) it
  computes task \dwords. The operations it applies to compute \dwords\
  are linear in $|w_{max}|$ so the complexity of the calculus is
  $\mathcal{O}(|V|+|E|*|w_{max}|)$.
\end{proof}

\subsection{Examples}
We first consider the deadline calculus of the example of
Fig. \ref{fig:dw-usefull}. To simplify, we consider that the durations
of the main node ($M$) inputs and outputs are null. The calculus first
computes $w_B=\drepeat{6}$ due to the deadline constraint on $o$. Then
it considers the precedence $A\precdiv{2} B$. We have $P(\Dclock 2)=2$
and $\diffops_{\Dclock 2}(T_B)=\drepeat{0.4}$. So, this precedence
imposes that $w_A\leq\drepeat{0.4}+\drepeat{6}-4$ ie
$w_A\leq\drepeat{2.6}$. $w_A$ was initialised to $\drepeat{4}$
first, so we have $w_A=min(\drepeat{4}, \drepeat{2.6}=\drepeat{2.4}$.

We then consider the example of the MSU. For abbreviation, we use $app$
for $applyCmd$, $bop$ for $basicOp$ and $fenv$ for $fromEnv$. We take
the following task durations: $C_{basicOp}=40$, $C_{applyCmd}=20$,
$C_A=30$, $C_B=10$, $C_C=20$, $C_D=40$, $C_E=10$, $C_F=30$,
$C_{fromEnv}=5$, $C_{toEnv}=5$. For every task precedence
$\tau_i\precany\tau_j$, let
$\cstr_{ops}(\tau_i,\tau_j)=\diffops_{ops}(T_j)+w_j+r_j-r_i-C_j$ (ie
$\cstr_{ops}(\tau_i,\tau_j)$ denotes the constraint relating $w_i$ to
$w_j$). The table below, gives the value of $S$, $\tau_j$, $\tau_i$ and
$\cstr_{ops}(\tau_i,\tau_j)$ at each step of the algorithm.

\[
\begin{array}{|l|l|l|l|}
  \hline
  S & \tau_j & \tau_i & \cstr_{ops}(\tau_i,\tau_j)\\
  \hline
  toEnv, A, D & toEnv & app & \drepeat{95}\\
  \hline
  app,A,D & app & bop & \drepeat{75}\\
  \hline
  A,D & A & B & \drepeat{470}\\
  \hline
  B,D & B & bop & \drepeat{460}\\
  \hline
  D & D & E & \drepeat{460}\\
  \hline
  E & E & F & \drepeat{450}\\
  \hline
  F & F & C & \drepeat{420}\\
  \hline
  C & C & bop & \drepeat{400}\\
  \hline
  bop & bop & fenv & \drepeat{35}\\
  \hline
\end{array}
\]

\subsection{Dynamic Deadline Computation}
\label{sec:dynamic-deadline}
The implementation of an EDF scheduler, as discussed in
\cite{buttazzo05}, can be performed on top of a generic priority based
operating system or from scratch. In both cases, the EDF policy requires
to compute the absolute deadline of each task instance at run-time. When
an instance $A[i]$ is released, its absolute deadline is computed as
$D_{A[i]}=R_{A[i]}+d_A$. If the scheduler is developed on top of an
operating system, task priorities are then reaffected depending on this
deadline. If it is developed from scratch, the task with the earliest
absolute deadline is directly scheduled.  

In our case, relative deadlines are not constant values but values that
differ from one instance to the next, defined by \dwords. \Dwords\ can
easily be handled by attaching a counter to each task that tracks the
instance number of the task. We then take the value corresponding to
this instance number in the deadline word. This is described in
Alg. \ref{alg:dynamic-deadline}. The overhead (a counter + an access to
a value in an array), when compared to classic EDF remains very
reasonable.

%\algblockdefx{Release}{EndRelease}{\textbf{Releasing task at R: }}{}
\algblockx[release]{Release}{EndRelease}{\textbf{At task release: }}{}
\algnotext[release]{EndRelease}
\begin{algorithm}
\caption{Dynamic absolute deadline computation for $\tau_i$}
  \begin{algorithmic}
    \State \textbf{Init:} $l\gets length(w_i); n\gets 0$
    \Release
    \State $d_i\gets w_i[n \mod l];$ $D_i=r_i+T_i*n+d_i$
    \State $n\gets n+1$;
    \EndRelease
  \end{algorithmic}
  \label{alg:dynamic-deadline}
\end{algorithm}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "compilation"
%%% End: 

